An AI Chatbot for Explaining Deep Reinforcement Learning Decisions of Service-oriented Systems

Deep Reinforcement Learning (Deep RL) is increasingly used to cope with the open-world assumption in service-oriented systems. Deep RL was successfully applied to problems such as dynamic service composition, job scheduling, and offloading, as well as service adaptation. While Deep RL offers many benefits, understanding the decision-making of Deep RL is challenging because its learned decision-making policy essentially appears as a black box. Yet, understanding the decision-making of Deep RL is key to help service developers perform debugging, support service providers to comply with relevant legal frameworks, and facilitate service users to build trust. We introduce Chat4XAI to facilitate the understanding of the decision-making of Deep RL by providing natural-language explanations. Compared with visual explanations, the reported benefits of natural-language explanations include better understandability for non-technical users, increased user acceptance and trust, as well as more efficient explanations. Chat4XAI leverages modern AI chatbot technology and dedicated prompt engineering. Compared to earlier work on natural-language explanations using classical software-based dialogue systems, using an AI chatbot eliminates the need for eliciting and defining potential questions and answers up-front. We prototypically realize Chat4XAI using OpenAI's ChatGPT API and evaluate the fidelity and stability of its explanations using an adaptive service exemplar.

==> approach.tex <==

\subsection{DeepRL4AS}
\label{sec:rl}
In general, RL aims to learn an optimal decision-making policy $\pi$ for when and which action to select in a given environment. 
Such a policy $\pi$ defines a mapping from environment states to actions.
Upon executing an action $A$ in a state $S$, the environment transitions to the next state $S'$ and awards a specific numeric reward based on a reward function $R(S, A)$.
An optimal policy $\pi$ is a policy that optimizes the cumulative rewards received~\cite{sutton_reinforcement_2018}.

Fig.~\ref{fig:mape-rl} illustrates how RL can be used to realize the adaptation logic by integrating RL into the MAPE-K reference model for adaptive systems (based on~\cite{MetzgerEtAl2022}).
Action selection of RL takes the place of the \textbf{A}nalyze and \textbf{P}lan activities of MAPE-K. 
The current state $S$ and reward $R$ are determined via the \textbf{M}onitor activity, and a chosen adaptation is performed via the \textbf{E}xecute activity.

\begin{figure}[htb]
  \centering
   \includegraphics[width=.5\columnwidth]{fig/MAPE-RL.pdf}
  \caption{Integration of Value-based Deep RL with MAPE-K}
  \label{fig:mape-rl}
\end{figure}


As XRL-DINE relies on a particular kind of Deep RL algorithms, so called value-based Deep RL, Fig.~\ref{fig:mape-rl} shows the specifics for this kind of algorithms.
In value-based Deep RL, the action selection policy depends on a learned action-value function, also called $Q$ function, $Q(S,A)$.
This action-value function thus represents the \textbf{K}nowledge in MAPE-K.
The action-value function gives the expected cumulative reward when executing an adaptation $A$ in state $S$.

Value-based Deep RL uses a neural network to approximate $Q(S,A)$~\cite{sutton_reinforcement_2018}. 
Based on $Q(S,A)$, a policy function determines for each given state, whether RL should exploit the current policy (i.e., choose the best action based on $Q$) or to explore new actions (e.g., by randomly selecting an action).




==> fundamentals.tex <==
\section{Preliminaries ((AM))}
\label{sec:fund}

\subsection{Explainability}
\label{sec:rl}
why questions, what kind ... \todo{see TAAS und MA Jan}


(1) what-questions (“What event happened?”), (2) how-questions (“How
did that event happen?”), and (3) why-questions (“why did that event happen?”). In contrast
to why-questions, both what-questions and how-questions are factual. In the context of self-
adaptive systems, a what-questions could be “what is the state of the system at a given point in
time?” or “what action did the adaptation logic choose at a given point in time?”. An example
for a how-question in the context of self-adaptive systems is “how did the adaptation logic adapt
the system at a given point in time?”. Since this thesis focuses on explainable adaptation tech-
niques aiming at supporting the user in understanding the adaptation logic, explanations mainly
focus on answering why-questions (e.g., see Chapter 3, especially Section 3.5).

explain here the different groups of questions (from the user study)
1--8

later then for each of the groups, we can use ...

A: 1
B: 2, 4, 5, 7 + 6 (eventuell)
C: 3 + 8 (eventuell zusammen)


\subsection{XRL-DINE}
\label{sec:xrl-dine}
summary



